Textile Taxonomy and Classification Using Pulling and Twisting

Identification of textile properties is an important milestone toward advanced robotic manipulation tasks that consider interaction with clothing items such as assisted dressing, laundry folding, automated sewing, textile recycling and reusing. Despite the abundance of work considering this class of deformable objects, many open problems remain. These relate to the choice and modelling of the sensory feedback as well as the control and planning of the interaction and manipulation strategies. Most importantly, there is no structured approach for studying and assessing different approaches that may bridge the gap between the robotics community and textile production industry. To this end, we outline a textile taxonomy considering fiber types and production methods, commonly used in textile industry. We devise datasets according to the taxonomy, and study how robotic actions, such as pulling and twisting of the textile samples, can be used for the classification. We also provide important insights from the perspective of visualization and interpretability of the gathered data.

==> old/conclusion.tex <==
\section{Summary and Conclusion}
{\red 
\begin{enumerate}
    \item We summarise the most meaningful results and the paper as a whole
    \item Future work can be an investigation of how an active second arm can help to enhance the exploratory primitives
\end{enumerate}
}

==> old/experiments.tex <==
\section{Experiments and Results}
{\red 
\begin{enumerate}
    \item Explain experiment details
    \item exe 1 Classification with Images alone is stupid
    \item Active manipulation is cool
    \item Combinarion performes the classification good
\end{enumerate}

}

{\mw 
This section is structured in the foillowing way:

First we will detail the experimental parameter used to perform all experiments,
next we perfomen classification experiments using only the macro vision data, showing that a robust classification is not possible. Followeing that we compare the two active manipulation strategyes (pull and twist) in regards to there signal usefullness for our classification tasks. Finnaly we combine both active and passive force/torque reading into a single framework and show what parts of the signal are used when performing the classification.

\subsection{Implementation details}
{\red here we can add all the numbers and hyper params from below
We need to agree on the final architecture and hyperparameters and framework first
}
}

{\al
\subsection{Experimental set-up}
Two Franka Emika Panda manipulators, two 6-axis Optofroce F/T sensors and a Logitech C920 video camera were made available for the project by KTH university. A 3D printed gripper was used instead of the Frankas' default ones to imitate as much as possible human's grip. {\red Don't know if the last comment should be mentioned since it goes beyond our purpose of keeping this set up easy to adapt in already existing pipelines} 

% \subsection{Training}
% {\blue changhe title of this section if you want to keep it}
% All experiments were performed with pytorch \cite{NEURIPS2019_9015}. To train the networks, the dataset was split into mini batches of X samples. Adam was chosen as optimizer which allowed to introduce L2 regularization through its \textit{weigth decay} parameter. BCEWithLogitsLoss class of pytorch was used as a loss-function,
% suitable for multiclass problems as it is a combination of Sigmoid activation function and Binary Cross Entropy loss.
% {\red Training/validation/test split}
% {\red How is validation performed?}
% {\red How we did the comparison}
% {\red How do we choose the best model? Early stopping?}
% {\red Which is the metric to compare the models? Classification accuracy?}
}

{\mw 
\subsection{Micro level vision classification}
We used ARCHITECKTURE to performe the classification task and got PERFORMANCE.
We investigate with Grad-CAM and se that NO MICRO LEVEL FEATURES ARE CONSIDERED




\subsection{Pull vs. Twist manipulation}
To evaluate if the different active manipulation strategy recover significant data we perform first an analysis into the datasets itself.

We show with t-SNE plots that the structure in twist is more favorable then with pull this gets colaberatet when doing a classification tasks on the active arm data with pull and twis and showing that twist performs higher -> the network can exploit the more infos.
We also show that twist datas individual readings (fx,fy,fz,tx,ty,tz) are more ritch by using a simple MLP to classify to what source a given signal belongs showing that it is easier to distingvish the twist data induvidual signals tbetter than the pull -> more deffrent information inside the sub signals.
To this aim we train a simple MLP with a single hidden layer and $1000$ nodes for  classification of all pull vs twist data individually. The result in Table {\red REF} show that {\red STUFF}

\subsection{Classification of Fabric Propertys}
as a final thing we show that we can indeed do garment classification on properties that are relevant for manipulation We train a ARCHITECTURE that uses twist active and passive and performes does the classification with RESULT. We also show with Grad cam what part of the signal as well as with sub-signals are responsible for the classifcation performance. If we need a bit more we can make another connection of pull vs twist at this point by showing that twist uses a more diverse set of signals?? (hopefully)



}



==> old/introduction.tex <==
\section{Introduction}
{\red 

We want the following paragraphs:
\begin{enumerate}
    \item Motivate why garment identification is important (we can allude to the difficulties of deformable object manipulation) and motivate why it is necessary to do it based on the structural properties for manipulation
    \item Exemplify with an assisted dressing scenario of how you would dress someone with hard VS soft/elastic material (potentially, swap the places of 1st and 2nd paragraphs)
    \item Make the case for combining vision and force readings $\rightarrow$ discredit fingertip sensors because money \textit{(maybe focus on how wrist mounted ones are more general-purpose cause microscopes came into play)} and because woven VS knitted is better distinguished by active manipulation over tactile one 
    % \item Draw parallels to humans (2 hands and eyes)
    % \item Nice picture top left with the setup (we use the panda model that's now the group logo :)
    % \item Make sure to cite our works where we can ;) \cite{lippi2020latent} 
    \item Emphasise that we consider this "active" component in order to get better readings (The "twisting" motion).  We motivate with what has been said in the previous paragraph.
\end{enumerate}
}

%{\mw 

%{\al I'VE WRITTEN THIS INTRODUCTION PART COMBINING MICHAEL IDEAS WITH MINE. IF YOU DON'T LIKE IT WE CAN STICK WITH WHAT MICHAEL HAS WRITTEN (}

%When human manipulate objects/ use tools or interact in any such way with there environment, a lot of prior experience is leveraged the instance humans interact with the object.

%For example before interacting with an object humans perform initial classification step first and foremost: "What is the object I'm about ti interact?"," What are it's attributes?". This internal questioning results in an estimate of the property's of the object, such as mass, material, and inherent structure. For example when packing a suitcase or bag we estimate the weight and fragility of items and pack accordingly. In this case we also often relay not only on vision but also on our sense of touch and {\red Is there a word for feeling the FORCE?} \cite{recognictionOfScenes}. This is especially important when handeling deformable objects.

%Manipulating and understanding deformable objects have enjoyed a recent rice in popularity in the robotics community~\cite{butepage2019visual},  {\red CITE 2-3 more}.  With garments and fabrics as an example of a highly deformable objects becoming more and more popular to Benchmark and showcase new advances in manipulation methods~\cite{garcia2020benchmarking}, \cite{lippi2020latent} {\red CITE 2-3x more examples}. 
%Most methods working with garments or the manipulation of other highly deformable object focus on the category classification in order to elevate the performance of there manipulation approaches~\cite{ziegler2020fashion} {\red CITE 1-2 more}. Other approaches like~\cite{petrik2019feedback} use Reinforcement learning and a feedback-based controller to deal with the many degrees of freedom that result from the often unobservable properties of the material determining it's underlying dynamics. {\al)}


Deformable objects are frequently encountered both in domestic and industrial robotic environments. The applications can span from food manipulation in a home kitchen, to large-scale garment sorting and recycling in a factory. 
In contrast to their rigid counterparts, the manipulation of deformable objects presents additional difficulties stemming from their materials' intricate dynamics that can affect their physical properties in an unpredictable way.

% When humans interact with their environment or manipulate objects and tools, prior experience is leveraged in order to determine how to carry out their task. Solely based on their vision and experience, they can perform an important classification step: ”What is the object I’m about to interact with?”, ”What are its attributes?”. This internal questioning results in an estimate of the properties of the object such as mass, material, and inherent structure. After establishing an initial estimate, they then rely on their haptic feedback to distinguish further properties of the object and expertly manipulate it, regardless of its rigidity. When packing a suitcase or a bag, for example, they estimate the weight and fragility of items and pack accordingly \cite{recognictionOfScenes}. The investigative process is especially important when handling deformable objects due to their uncertain shapes and poses during manipulation.
{\im \textit{ Short description of how the structure affects the dynamics. Not too much detail, that goes in the specialized section. Conclude with why both vision and force are needed.}} Fabric dynamics during manipulation are affected by its structural properties. In an assisted dressing scenario, the elasticity, thickness and weaving of the material dictate how to tune the controllers to efficiently complete the task, with no damage to the human or the garment. These properties are very difficult to determine visually, or through haptic exploration without very specialized equipment. To circumvent this, we can complement the visual information with wrench signals from {\red exploratory/torsional/active primitives} that are designed to showcase the material's properties. 
 {\red \textit{and then we talk about how the motions do that (aka stretching helps vision for weaving and force for elasticity.  twisting helps vision for thickness and force for thickness and elasticity) and present the proposed method.
 We also say that part of the investigation is the effect of the bimanual setup}
}

% However, the perplexity of human perceptual skills is difficult, and often costly, to emulate solely based on haptic or visual feedback. 
% % Inspiration to tackle this problem can be drawn from how human brains solve this task.
% During object recognition, the human brain jointly extracts information from different senses, also called \textit{modalities} \cite{multimodal_learning_survey}. Haptic and visual signals are processed in a multi-sensory fashion by learning a shared representation of these data \cite{humanCrossmodalIdentif}.  Therefore, coupling these sensory modalities provides more information which helps boost the performance in a variety of robotic tasks \cite{deepLearningVisualHaptic}.

Learning a combination of visual and physical properties for deformable objects has showcased a recent rise in popularity in the robotics community \cite{butepage2019visual}, \cite{recognictionGrasping}. Concretely, garments and fabrics are an example of highly deformable objects which are becoming more and more popular to benchmark and showcase new advances in manipulation methods \cite{garcia2020benchmarking, perceptionAssistiveManip, lippi2020latent}. Most manipulation methods working with clothes, or other highly deformable objects, focus on the garment's category classification in order to improve the performance of their manipulation approaches~\cite{ziegler2020fashion, visionForceControl}. Other approaches like~\cite{petrik2019feedback, miltumodalvision}, use Reinforcement learning and a feedback-based controller to deal with the many degrees of freedom that result from the, often unobservable, dynamic properties of the material.



 



% {\al To cope with the tough challenge of understanding the nearby environment, robots require intelligent algorithms that provide them with the ability to interpret all the incoming information and distinguish objects' common feature. Humans, for example, before interacting with objects rely on their experience leveraging vision and their a priori knowledge to do an initial classification step first and foremost: ”What is the object I’m about to interact?”,” What are its attributes?”. This internal questioning results in an estimate of the properties of the object such as mass, material, and inherent structure. The act of manipulation instead, often rely not only on vision but also on humans' sense of touch and feel of the object. Packing a suitcase or a bag, for example, we estimate the weight and fragility of items and pack accordingly \cite{recognictionOfScenes}. This is especially important when handling deformable objects due to their uncertain shape and pose that can assume.}




{\im \textit{Tentative text that will change when the results are out: }
To distinguish the material dynamics in a more efficient {(\red efficient in which sense?cost?)} way, we propose a framework that uses an overhead camera, as well as the more common wrist-mounted force/torque sensors, as shown in Fig.~\ref{fig:system}. 

Our experiments confirm that in order to correctly classify a number of similar-looking, but dynamically differently behaving fabric materials (such as wool, cotton, denim, etc.) the combination of visual and force/torque readings is beneficial. 
Furthermore our framework shows that how we interact with the material when acquiring the sensor readings matters, i.e. the way we stretch and pull the fabric, influences the quality of our prediction, similar to the exploratory movements a human employs to estimate fabric material with a higher certainty. Finally, we show that the quality of the sensory input is important and argue that such a system can have enormous benefits when implemented in a garment/fabric manipulation pipeline.

In detail our contributions are:

\begin{itemize}
    \item Framework to identify garment materials using wrist mounted force/toque sensors and overhead camera
    \item Insights into importance of sensor quality %(Franka vs optoforce)
    \item Insights into importance of "active" data gathering %("twist" vs "no twist")
    \item Combined dataset of sensor readings for XX garment materials
\end{itemize}
}

 \begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/system_100.png}
  \caption{{\mw System overview: Two 7 DoF Manipulators equipped with force/toque sensors mounted on the wrists, twisting and pulling a piece of fabric. On top a camera looking to capture the deformation visually.}
   }\label{fig:system}
\end{figure}





==> old/method.tex <==

% {\red 
% I'm not convinced with calling the main section method as we don't  really have a Method ... how about:}

{\mw
\section{System Overview}
Our system as shown in Fig.~\ref{fig:system} consistes of two 7 DoF manipulator that hold a pice of fabric between them. The \textit{passive} arm does not move during the manipulation of the fabric, while the \textit{active} arm can performe diffrent manipulation stratgys. A overhead camera is mounted on top to observe the visual deformation of the fabric during manipulation.

A pice of fabric is then put betweent the two armas and the active arm statrs the manipulation process resulting in three destinc collected datasets: $\mathcal{D}_a$, $\mathcal{D}_p$, $\mathcal{D}_v$ wich are the \textit{active} arm, \textit{passive} arm, and vision data respectivly. {\red we could add the details about the sensors in this block ...}

We destinquese between two different active manipulation strategy's:

\noindent
\textbf{Pull manipulation:} In this case the \textit{active} arm performas a simple pull motion, in detail it {\red XX here we can now fill the details about the pull controler}
This results in the three datasets: $\mathcal{D}_a^{pull}$, $\mathcal{D}_p^{pull}$, $\mathcal{D}_v^{pull}$ 

\noindent
\textbf{Twist manipulation:} The second case a more involved twist motion is performed because {\red JUSTIFY and write details}
This results in the three datasets: $\mathcal{D}_a^{twist}$, $\mathcal{D}_p^{twist}$, $\mathcal{D}_v^{twis}$ 

}


{\im \textit{Subsections Datasets and Preprocessing have been moved from Section "Motivation"}}
\subsection{Datasets}

{\red ?QUESTION? Of course I have to mention how we collect the data, but how deep do I need to go with the tasks explanation? By now we'd like to justify this part in the method section, I might just refer to that section}

Due to the lack of datasets suitable for our purpose, we framed a data collection procedure to provide us with the required measurements for the experiments. We took into account  X different garment materials {\blue there must be an explanation of why we have chosen to consider these classes(follow Dani's suggestions)}. For each class, XX samples were cut into 40x17 rectangles and they were labelled corresponding to the fabric they were made of.  Each one of them was explored Y times both for the pulling and twisting (EXPLAIN BETTER...) {\blue pulling and twisting, brief explanation and refer to the corrispective section}.  {\red Understand how many times you want to repeat each experiment, I would start with three, no more...}
{\blue here just introduce and briefly explain the distinction between pulling ad twisting}

{\blue Which are the senses taken into account? Use this as connection to the measuremetns that we include in the dataset}

The different processing of cotton to obtain denim modifies the dynamics of the latter. The percentage of cotton contained, therefore, is less relevant {\blue brief explanation why we distinguish btw cotton and denim. could be extended}.



The measurments are the results of different exploration porcedures that aim to detect as much as possible the intricate dynamics of fabrics as will be explained in section(blahblah)

We ended up with two dataset of ZZ elements.


\subsection{Preprocessing}
{\blue you shuld mention the shape of raw data if you want people to fully  understand your preprocessing phase}
{\red I still have to decide if to incorporate this section in the dataset one or not. If you hava any suggestion is welcome :)} {\im I suggest to keep them separate initially and have the Dataset only describe the materials. If there are space issues, you concatenate them.}
Each signal was downsampled to {\red 150?} samples, where each one of these samples was obtained by averaging all the values removed. Furthermore, these signals have been normalized {\blue explain better this normalization phase pls}. {\blue Here explain the concatenation of the signal coming from the same sensor.} In order to construct a sample meaningful for classification of fabric materials, the 6 signals collected from each sensor ($F_x$; $F_y$; $F_z$; $T_x$; $T_y$; $T_z$) were concatenated along the axis opposed to the time axis to form a matrix of dimension 150x6.
For the images, the stream of {\red 150?} images for each experiment was downsampled
to {\red 20?} frames. Each image was converted into gray-scale and cropped to the
size of interest {\red (90x150 pixels)}. The position of the crop was chosen to let the
network focus on the wrinkles created on the fabric during the manipulation task.
{\blue Should I put here the structure of an input sample? } To take into account the image 
ow along with the whole experiment, a single sample was built as a 3D matrix of dimension 20x90x150, where the first dimension corresponds to the time channel. This choice was motivated by the interest in capturing the dynamics of the fabric by extracting features that consider also the time axis.






%-------------------------------- Can be reused for the previous section if need be
% \section{Method}
% {\red 
% \begin{enumerate}
%     \item Justify the employed method as well as the resulting architectures
%     \item Motivate the "twist" and explain how we will evaluate the results etc (also grad cam usage for 1D)
%     \item present full framework
% \end{enumerate}
% }


% {\red brief introduction by recalling the goal of this paper.}
% GOAL..
% The problem : Endowing robots with the capability of distinguish garments material is a difficult task. Vision itself is not enough as clothes often share similar feature even though they are of different type. 

% Therefore we appoached the problem.. (from which perspective?)

% To accomplish this...

% {\blue here start describing the problem and the challenges, from the problems get to the sensors and why we used them to investigate our problem. from the sensor (or maybe even before) the exploratory procedure has to be intorduced and motivated (but for sure the detailed definition has to be done ) Then it has to be intoduced the concept of the multimodal analysis, the fact that vision is not enough and multisensory signals (if they are complementary) are helpful for the classification }
%--------------------------------

\subsection{Exploratory procedures}
{\red Still not sure that this is the correct position of the section}
{\im It again depends on what you are selling with this work. If you want to say that "hey, the way i manipulate the fabric plays a role" then this stays in the method. }
{\blue\textit{You should start with a more precise definition of what is an exploratory procedure}}
With the term \textit{exploratory procedure}, in this work we refer to a manipulation action intended to capture the different dynamics and properties of the fabric materials. It includes two exploration
procedures: pulling  and twisting.
{\blue Twisting is important because we choose to use sensor on the wrist (if they were on the fingertips of course it would be non sense) and they let us perceive another "dimension" of the dynamics of the fabric. Just pulling we do not sense the torques and our hypothesis is that this is a good point do distinguish not only the materials but also its weaving and finish...}

{\blue define better the pulling and twisting procedure}
{\blue why twisting is so interesting }
Although jeans and cotton t-shirts are mostly made of the same material, the response they provide to the twist is significantly different. {\blue explain more btw differences of pulling and twisting and why we do expect more information form pulling}  {\red In the experiments we need to verify our hypothesis about "twisting more relevant" }

To differentiate the movements of the arms, the left one was kept still during the whole data collection procedure. The main operation has therefore been carried out by the right arm, which was simultaneously performing the following actions:

\subsection{Classification Architecture}
{\im \textit{The final architectures can go here.}}
\paragraph*{\textbf{Signal Classification}}
The model architecture for signal classificaiton is composed by 4 set of interleaving 1D convolutional layers which output respectively 24, 12, 8 and 4 filters. The kernel size is 5 with stride 2 for all the filters. Batch normalization and ReLU where used between each convolutional layer. The output of the last convolutional layer serves as input of a fully connected layer which outputs 4 neurosn corresponding to the 4 classes. The choice of using 1D convolutions has been done to \textit{group} channels as in \cite{deepLearningVisualHaptic}, where a \textit{channel} corresponds to each force or torque signal of the sensors. Grouping means instead that each signal does not interact with the other ones inn the network. By means of this technique, interactions between different signals are not learned until the first fully connected layer.
\paragraph*{\textbf{Image Classification}}
The classification of images has been carried out by means of a CNN. The networkis composed of 4 2D-convolutional layers that output respectively 12, 8, 4 and 4 filters. The size of the kernels is 5 and the stride has been chosen equal to 2. As done for the network signal , Batch normalization and ReLu have been used among the convolutional layers.The features learned by the
convolutional layers are flattened into a 48-long vector in order to feed it into a fully connected layer which outpts 4 values relative to the 4 classes.

\paragraph*{\textbf{Multimodal Classification}}

% {\blue Justification of multimodal architecture from multi sensory modality of the brain?}


{\blue Explain the multimodal archiecture which is the result of the combination of unimodal architecture where the las fully connected layer was removed to perform late fusion. (LATE FUSION HAS TO BE MENTIONED) (THE PAPER THAT DO THE SAME HAS TO BE CITED)}
The first choice made about the multimodal classification was to adopt the late fusion technique to combine the representations learned from each modality as in \cite{deepLearningVisualHaptic}. This architecture requires that the streams responsible for each modality coincide with the unimodal networks described in the previous sections up to the classification layers. Therefore, the input of the multimodal network is composed of both the signal and the image datapoints coming from the same experiment. The outputs of these models correspond to the learned features. Each of them is composed by 48 neurons that are concatenated and fed to a fully connected layer responsible for the classification of the materials. ReLU has been chosen as activation function for the last fully connected layer.

{\blue Explain how we perform comparison btw unimodal and multimodal to see effectiveness of multimodal network }

%--------------------------------
% {\red MW: If we have the system overview we can have a seperate chapter for the architecture}


% {\mw 
% \section{Classifiaction Architecture }
% In this section we descipe first the induvidual as well as the multimodel architecture used for fabric material classification.
% \subsection{Force/Torque Classification}
% {\red FILL achitecture for f t thing}

% \subsection{Vision Classification}
% {\red I don't like the section names}

% \subsection{Multimodel architecture}
% combo of the other 2 with final things combined.

% }
%--------------------------------

==> old/problem.tex <==
\section{Motivation}
{\im \textit{Should this be called motivation, preliminaries, background? The name has to change depending on which subsections end up here.} }


{\al
{\red Formalise the problem of garment classification}
% \subsection{Garment classification}
The problem of classifying clothes material can be approach from many point of view. They could be classified according to the textile structure such as woven or knitted. Texture  as well  is a visual property useful to distinguish garments. From an engineer perspective, instead, what would be interesting are the physical characteristics like thickness, weight and elasticity. All these garment analysis could mislead from the main purpose, which is material classification. Nevertheless, the combination of these complementary features brings to a well-defined distinction between garment materials such as cotton, denim, wool, etc...{\red Ask Dani how this could be improved and defined better and which are our classes}
The challenges that have to be faced mostly concern the deformable nature of fabric. Slightly changes in the conditions in which the manipulation takes place may lead the same garment to behave differently. The same could happen if what sets a particular type of fabric apart from another one is its weaving and finish. 
{\red missing a good conclusion for this paragraph}
{\im Something like "In the following section we illustrate these difficulties and propose solutions based on blah blah?"}
}


\subsection{Fabric Properties for Manipulation}

{\red Is it knit or knitted? (It's actually both in perfect participle. You can decide which one sounds better)}

All fabrics can be characterized by two components: fiber material and fiber construction. The fiber material can be either natural (cotton, wool, silk) or manufactured (nylon, lycra, acrylic). The fiber construction can divide fabrics into three classes: woven, knitted or non-woven. The knitting construction can be further characterized as either weft or wrap. 

Woven fabric is usually produced by using two sets of yarn, while knitted fabric employs a single set. To produce woven fabric, the yarn is interlaced, as opposed to knitting where it is interloped, see Fig. \ref{fig:woven_VS_knit}

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{figs/draft_weave_VS_knit.jpeg}
    \caption{Woven fabric yarns are interlaced, while knit fabric yars are interloped.}
    \label{fig:woven_VS_knit}
\end{figure}

Due to its construction, woven fabric is often hard and nonelastic, allowing it to hold creases well, and can be only stretched diagonally. It is commonly used to produce garments such as shirts and denim pants. 
On the other hand, knitted fabric is soft and can be stretched in all directions, making it wrinkle-resistant. Common applications are t-shirts or polo shirts.


These differences produce vastly diverse dynamics for manipulation. For example, both denim pants and a polo shirt can be made with 100\% cotton that has been woven or knitted respectively. In an assisted dressing scenario, the differences in pliability and stretch of the fabric would require very different tuning of the controllers or grasping strategies. 
 





{\red 
Here we explain why we label the samples the way we do by explaining what weaving etc is and that same materials can have very different properties. We showcase this with a Marco and micro image showcasing the weaving. I imagine a figure where we see 2 similar looking cloth pieces on the Marco level and the microscope gives us a very different view showing that they are diff-rent and will behave dynamically different (FIG \ref{fig:draft1} 


}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figs/draft_fabrics.png}
    \caption{Fabric can look the same on the macro level, but very diffrent on the micro level (right). The diffrent weaving styls wiht the same material determine the dynamical propertys that are important when manipulating fabric.}
    \label{fig:draft1}
\end{figure}

{
We in addition show that the microscope labeling is also sensible given the recorded force/torqe readings with a simple t-snes comparision plot: Fig \ref{fig:draft2}
}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figs/draft_lable_diff.png}
    \caption{t-Sne plots of the same recorded force toqe readings but diffrent labels. Left we see the lables following the material of the fabric, while right it follows the microscope analysis. We onserve a lot}
    \label{fig:draft2}
\end{figure}





\subsection{Multimodal Perception}
{\red Here we can explain/motivate why multimodal perception}

{\im Fabric material identification based on a single modality is a considerably difficult task as the material's preprocessing might alter its properties.  Vision-based approaches can be sub-optimal since it is possible that samples from
the same material behave similarly but look nothing alike, or that two samples that look the same, are from different materials. On the other hand, relying only on force sensing can be challenging due to the fabric's intricate dynamics. For example, a woven and a knitted fabric can have the same elasticity and response when stretched, making them distinguishable only through vision. {\red all of the above may need tweaking to be more accurate.}

These observations are summarized in Fig. {\red aaa}. Concretely, the top row consists of image  samples from  {\red class1, class2 and class3}, while the bottom row presents {\red yada yada signals}. 

\textit{I am imagining 3/4 samples of images that push the following points across: Fig 1 and 2 look very alike but are different materials, Fig 1 and 3 look very unlike but are the same. Then the bottom row has either two t-sne or mean and std of the above classes that hopefully do not give too much help and then the last image is the t-sne of the multimodal guys which should be better. }

{\red Say again that stretching is good for seeing elasticity and (potentially) weaving and then we add twisting to that to also see/feel thickness?}
}

{ \mw 
% Fabric material identification is a challenging task, as fabrics can have the same material but look vastly different making classification based on optics soly a difficult feat.
% The idea behind mixed data classification is to leverage different data modalities to improve the overall classification performance.
For the specific case of garment material classifications we consider three seperead input sources: \emph{i)} Force/Torque readings from an optoforce{\red CIT} sensor mounted on the writs of an \textit{active} arm. \emph{ii)}  Gray-scale images from an overhead camera looking at the considered sample. \emph{iii)} Force/Torque readings from an optoforce{\red CIT} sensor mounted on the writs of an \textit{passive} arm (See Fig.~\ref{fig:system}).

The idea of the mixed data classifiacion is to combine the complementary information present in the different sensors. The vision gives insight into the deformation that is visible on a marco level during the manipulation of the fabric{\red MW: we have garments and Frabric should we stick to 1?} {\im fabric/material to me are ok, garment hints at differences in their form}. The \textit{passive} arm recoreds the effects of when the material is pulled with a constant counter force, and the \textit{active} arm records the result of pulling or any other active manipulation to enhance the classifaction capability of the signal by perfroming a \textit{twising} motion for example.

The considered problem therforw boils down to answering the following questions:
\begin{enumerate}
    \item Can Fabric material be reliable identifyd by combining Force/Torque and visual information)
    \item Do different active manipulation strategies {\im exploratory primitives?} make it easier to performe acurate classifiactions of Fabric material?
\end{enumerate}

To answer this questions we collect four diffrent datasets, two for diffrent manipulation stratgies f the active arm and one each from the camera and the passive arm. {\red \textit{See section blah blah for details}}


}




==> old/related_work.tex <==
\section{Related Work}

% {\red 
% \begin{enumerate}
%     \item List related work for classification
%     \item Material classification in particular
%     \item Combination of sensory input
%     \item Combination of sensory input for material classification in a robotic context
%     \item Highlight differences/advantages of our approach 
% \end{enumerate}
% }

% {\im I propose the following narrative : }

% {\im  In \textbf{Introduction}, 1 paragraph for very general mention of classification tasks in robotic manipulation (object detection, event detection, object classification) --item 1.   }

% {\im In \textbf{Introduction}, 1 paragraph for multimodal perception --item 3. }

% {\im In the last \textbf{Introduction} paragraph, really sell the challenges of deformable materials/fabric to work as a segue to the related work. \cite{perceptionAssistiveManip}} 

% \im Start related work with item 2. Conclude with a sentence of how some idiots have either only rigid or \textit{slightly} deformable objects and you are working with much more difficult ones. The other idiots that do deformable objects use bad/expensive sensors etc.
% Vision based \cite{spectroscopy0, CNNMaterialRecognition, recognictionGrasping}. 

Material identification in robotics has been treated with three main categories of approaches: contact based, non-contact based and a combination of the two.

In the first category, Kerzel et al. \cite{MultiChannelNN} utilized OptoForce 3-Axis optical force sensors, a dome-shaped device which mimics a human fingertip. Using lateral and vertical motions, they classified materials based on the vibrations between sensor and object, reaching 98\% accuracy. In a similar manner, Kerr et al. \cite{materialTactileSensing}, employed a SynTouch Biomimetic Tactile (BioTac) fingertip sensor that provides measurements of low and high-frequency vibrations, fluid pressure, temperature and deformation of the finger surface. The combination of these sensing modalities, outperformed human participants in a material classification task. Both works achieved impressive results, potentially due to the richness of the signals considered. However, these sensors come at a higher cost than the more general-purpose force sensors, which should be taken into account. 
Apart from  the specialized fingertip sensors, there are more tools that rely on physical contact to provide local observations. Different possibilities include measuring the torques exerted at the actuators of the robot as in Gemici et al. \cite{Gemici2014}, or the external forces measured by a wrist-mounted force/torque sensor, as done by Paraschidis et al. \cite{1990}. {\im Find maybe a newer one for the sensor based?}


% The measurements gathered performing lateral motions over the object, allowed the authors to categorise materials based on vibrations caused by the friction between sensor and surface. They achieved 98\% accuracy  employing a multi-channel 1D CNN. One convolutional processing path was intended to extract spectral features of sensory data gathered from a lateral exploration of the object, while the second feed-forward path processed data coming from the pressure exploration procedure. 

% The even more complex SynTouch Biomimetic tactile sensor (BioTac) mimicsas well the sensory capabilities of a human fingertip \cite{materialTactileSensing} . It records low and high-frequency vibrations, fluid pressure, temperature and deformation on the artificial finger surface. The combination these haptic data allowed to overcome humans'  classification capabilities. 



In the non-contact category, vision-based techniques have been explored in material identification to distinguish object characteristics such as type, shape or texture \cite{CNNMaterialRecognition}. Specifically, Corona et al. \cite{recognictionGrasping} proposed a hierarchy of three CNNs with different levels of specialization to carry out garment identification. {\im what is the main diff with that guy?}. Furthermore, Erickson et al. \cite{spectroscopy0} explored a non-contact technique for material estimation using spectroscopy with an intricate sensing device that provides information about the interaction between electromagnetic radiation and matter. {\im Do we need more citations here?}


While vision is appropriate for capturing characteristics of the materials' appearance, haptic and force sensing are more helpful for characterizing physical properties. Thanks to the complementary nature of these modalities, their combination has proven to be beneficial for material classification. Gao et al. \cite{deepLearningVisualHaptic}, employed a BioTac sensor to infer haptic adjectives and improved object classification by coupling it with visual predictions. By combining the two modalities into a multimodal CNN model, they obtained a classification accuracy of 86\%, that surpassed the models based on either modality. In an extension of their previous work, Erickson et al. \cite{spectroscopy} introduced a multimodal sensing technique that leverages spectral measurements and close-range high-resolution texture defining imaging. For each modality, a separate representation was first learned and consequently combined into a shared representation to classify the materials of household objects. {\im And here we add what is similar/inspired by them or what is different.}

{\red Maybe a section about multimodal learning?}

{\red TODO: Add works on
\begin{enumerate}
    \item computer vision for fabric-related stuff
    \item assisted dressing and HRI
    \item folding etc in robotics
\end{enumerate}
}

% {\red \cite{visionForceControl} in my opinion shuldn't go here since it's about control and not classification. It could go in the introduction.}
% {\red About \cite{miltumodalvision}, it's more about multimodal representation, but could be integrated to explain multimodal architectures such as \cite{3DCNN}.}





% Vision is able to acquire characteristics described by the appearance of the materials, while physical adjectives are better characterized by signals such as
% force and torque. 
% As these two modalities provide complementary information about object properties, joining them in the classification task helps increase the accuracy of each single modality.


% {\al In fact, in \cite{deepLearningVisualHaptic} the authors improved object understanding coupling vision predictions with haptic adjectives inferred through a BioTac sensor. They transferred learned weights form visual and haptic CNN models to a multimodal network obtaining a 86\% accuracy in haptic classification showing that multimodal architecture can leveragethe strengths of each modality.
% Erickson et al. extended their previous work in \cite{spectroscopy} introducing a multimodal sensing technique that leverages spectral measurements and close-range high-resolution texture defining imaging. For each modality {\red I defined in the introduction the concept of modality}, a separate representation was first learned and consequently combined into a shared representation, to classify materials of household objects. }




% {\al Vision allows differentiating objects characteristics such as type, shape or texture, that can be meaningful to infer the material of which they are made. 

% {\red  \cite{CNNMaterialRecognition}}}
% Corona et al. \cite{recognictionGrasping} proposed a hierarchy of three CNNs with different levels of specialization to carry out garment identification.





% {\al Kerze, Ali et al. \cite{MultiChannelNN} worked with OptoForce 3-Axis optical force sensors, a dome-shaped device which mimic a human fingertip. The measurements gathered performing lateral motions over the object, allowed the authors to categorise materials based on vibrations caused by the friction between sensor and surface. They achieved 98\% accuracy  employing a multi-channel 1D CNN. One convolutional processing path was intended to extract spectral features of sensory data gathered from a lateral exploration of the object, while the second feed-forward path processed data coming from the pressure exploration procedure. The even more complex SynTouch Biomimetic tactile sensor (BioTac) mimicsas well the sensory capabilities of a human fingertip \cite{materialTactileSensing} . It records low and high-frequency vibrations, fluid pressure, temperature and deformation on the artificial finger surface. The combination these haptic data allowed to overcome humans'  classification capabilities.  }

% Force based \cite{1990}.

% {\al Fingertip sensors, however,  are not the only tools that rely on physical contact to provide local observations. Different possibilities include measuring the torques exerted at the actuators of the robot, or resort to a wrist-mounted force/torque sensor. \cite{1990}}

%  Start multimodal perception paragraph with something along the lines of "we need both touch and vision" and describe item 4. \cite{spectroscopy, visionForceControl, miltumodalvision, dressingDynamics, 3DCNN, deepLearningVisualHaptic}.










==> old/todos.tex <==
{\red 
\section{TODOS}

% \begin{itemize}
%     \item Setup experiments paper version:
%     \begin{itemize}
%         \item Lower camera for higher def vision images
%         \item Finalise "twist" and "no twist" controller
%         \item Prepare Garment material samples
%     \end{itemize}
%     \item Setup training and evaluation pipeline on Mordor:
%     \begin{itemize}
%         \item raw rosbags $\rightarrow$ prepared pkl file
%         \item Training procedure on Mordor
%         \item Evaluation and explainable components (Grad cam for 1D and 3D)
%     \end{itemize}
%     \item Collect data
%     \begin{itemize}
%         \item set up material i of XX
%         \item perform "no twist" $\rightarrow$ reset position (don't release)
%         \item perform "twist" $\rightarrow$ reset position (don't release
%         \item Do previous 2 steps XX times
%         \item set up next material sample
%     \end{itemize}
%     \item Design/test individual architectures on Mordor/RPL cluster
%     \item  { \textit{Write Introduction /related work (can be done before experiments are there)}} Remove unnecessary paragraphs and duplicates from Intro
%     \item Write Problem/ datasets collection (can be done as soon as we collect data)
%     \item Write Method (need final models before starting
%     \item Write Experiments and results (need all the results)
%     \item polish writing (last step)
     
% \end{itemize}

\textbf{General Context:} 

\textit{update 19 Feb}

For manipulation, it is important to classify the fabric based on its (stretching) properties, not its material. This is because the dynamic properties of fabric during its manipulation are mostly affected by its construction.
% The main point we want to show is that it is useful to classify the Fabric properties for the purpose of manipulation! Our point is That the dynamic properties of the fabric (which is the important part when manipulating them) does come not simply from the material but from the way the material is woven.
We will have a section explaining the process of constructing different fabrics and show the difference of woven/knitted.
We will also describe the problem of macro images of the fabric (no construction details visible) with microscope images where the technique is visible. 

We want to investigate two types of actions that help us identify the materials. We want to do this based on forces to make sure the subsequent tasks can be executed properly. We focus on the manipulation aspects, which makes the images not as useful and we show that they can't properly classify everything. (they also depend on lighting conditions which is bad)
We argue that with just the wrist sensors we can classify the fabric in classes determined by the microscope.

We exemplify everything through the assisted dressing paradigm. 

\textit{We show that an "active" stretching (twisting) gives us a richer sensory read to be used for classification than simply pulling.
}
Experiments: 
\begin{itemize}
    \item We show that a purely vision-based classification is not sufficient and that it does not take into account the micro-structure of the fabric. We can potentially show that any learning success stems from artefacts that are exploited (color, structure, etc) 
    \item We show the advantage of "active manipulation" by analysing the raw data with t-SNE plots as well as performing classification on the individual signals (active VS passive) {\al this is something that goes well with the idea of exploring different ways of exploring materials}
    \item We propose an architecture that combines both (active and passive) arm readings and is able to perform high quality classification of fabrics with regards to their structural properties.
\end{itemize}

We need to convey 2 important concepts:

1) Classification just for material is not enough when the goal is better manipulation $\rightarrow$ our go-to example is assistive dressing where the behavior of the clothing changes a lot given the PROPERTIES (not the material) of the fabric and different materials can have the same properties, while same materials (woven cotton/denim vs knitted cotton) are the same but behave very differently.

2) The active manipulation enhances the information quality of the signal making classification easier, this ties into the advantages of wrist mounted sensors over fingertips and such as we want to classify given the properties that emerge when the fabric is manipulated (stretched/ twisted etc). This will be supported by a section on the taxonomy of fabric. 






}
